Re-recognized universality of Kozai oscillation on three-body dynamics

In 1962, Yoshihide Kozai reported his findings on the secular dynamics of asteroids moving in orbits with high inclination and eccentricity. In contrast to the classic understanding of the stability of planetary motion in the solar system, Kozai showed that asteroids can significantly change their orbital shape over a long timescale in an oscillatory manner between nearly circular orbits and highly elliptic orbits. An anti-correlated variation between orbital inclination and eccentricity characterizes this oscillation. The importance of Kozai's work in understanding the dynamical evolution of various systems was recognized decades later, including the fields of irregular satellites of planets, Oort Cloud, extrasolar planets, binary star systems, type Ia supernovae, planet climate, merging black hole systems, and so on.

==> babelbst.tex <==
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from babelbst.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file merlin.mbs.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% Copyright 1994-2004 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2004/02/09 4.13 (PWD, AO, DPC)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\iflanguage{finnish}{\input{finnbst}}{
  \iflanguage{english}{\input{englbst}}{
    \iflanguage{swedish}{\input{swedbst}}{
      \iflanguage{germany}{\input{germbst}}{
        \input{finnbst}
      }
    }
  }
}
% \endinput
%%
%% End of file `babelbst.tex'.


==> englbst.tex <==
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{and}                \def\bbletal{et~al.}
\def\bbleditors{editors}        \def\bbleds{eds.}
\def\bbleditor{editor}          \def\bbled{ed.}
\def\bbledby{edited by}
\def\bbledition{edition}        \def\bbledn{edn.}
\def\bblvolume{volume}          \def\bblvol{vol.}
\def\bblof{of}
\def\bblnumber{number}          \def\bblno{no.}
\def\bblin{in}
\def\bblpages{pages}            \def\bblpp{pp.}
\def\bblpage{page}              \def\bblp{p.}
\def\bbleidpp{pages}
\def\bblchapter{chapter}        \def\bblchap{chap.}
\def\bbltechreport{Technical Report}
\def\bbltechrep{Tech. Rep.}
\def\bblmthesis{Master's thesis}
\def\bblphdthesis{Ph.D. thesis}
\def\bblfirst{First}            \def\bblfirsto{1st}
\def\bblsecond{Second}          \def\bblsecondo{2nd}
\def\bblthird{Third}            \def\bblthirdo{3rd}
\def\bblfourth{Fourth}          \def\bblfourtho{4th}
\def\bblfifth{Fifth}            \def\bblfiftho{5th}
\def\bblst{st}  \def\bblnd{nd}  \def\bblrd{rd}
\def\bblth{th}
\def\bbljan{January}  \def\bblfeb{February}  \def\bblmar{March}
\def\bblapr{April}    \def\bblmay{May}       \def\bbljun{June}
\def\bbljul{July}     \def\bblaug{August}    \def\bblsep{September}
\def\bbloct{October}  \def\bblnov{November}  \def\bbldec{December}


==> pream4.tex <==
%% The amssymb package provides various useful mathematical symbols
\usepackage{amssymb}
%% The amsthm package provides extended theorem environments
%% \usepackage{amsthm}


%%%
%%% Comment over more than a line - this can come much earlier than other defs
%%%
\long\def\comment#1{}
\comment{
   Usage:
     \comment{ comments....}
}

%%% The (classic) Dennou style
\makeatletter
\def\DD{\@ifnextchar [{\D@D}{\D@D[]}}
\def\D@D[#1]#2#3{\frac{d^{#1} #2}{d #3{}^{#1}}}
\def\DP{\@ifnextchar [{\D@P}{\D@P[]}}
\def\D@P[#1]{\@ifnextchar [{\D@Pi[#1]}{\D@PD[#1]}}
\def\D@PD[#1]#2#3{\frac{\partial^{#1} #2}{\partial #3{}^{#1}}}
\def\D@Pi[#1][#2]#3#4{\left( \frac{\partial^{#1} #3}{\partial #4{}^{#1}}\right)_{#2}}
\makeatother
\def\DPsd#1#2#3{\frac{\partial^2 #1}{\partial #2 \partial #3}}

%%%
%%% (Sort of) Bug fix for lineno style.
%%%           Put it before \usepackage[switch]{lineno} !
% http://lambtani.hatenablog.jp/entry/2016/04/26/193817
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
  \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
  \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
  \renewenvironment{#1}%
     {\linenomath\csname old#1\endcsname}%
     {\csname oldend#1\endcsname\endlinenomath}}% 
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}}%
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
}
%\usepackage[switch]{lineno} % For 2-column
%\usepackage{lineno}         % For 1-column
%\linenumbers

%% The lineno packages adds line numbers. Start line numbering with
%% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
%% for the whole article with \linenumbers.
%% \usepackage{lineno}
\usepackage{lineno}
%\linenumbers*[1] % Never do it here - Do it on each file!
%\linenumbers

%%%
%%% xcolor - used quite often
%%%
\usepackage{xcolor}

%%%
%%% grahicx - choose your option by either of
%%%
% \dvipdfmgraphicxtrue
%  or
% \dvipdfmgraphicxfalse
%%%
\ifdvipdfmgraphicx
  \usepackage[dvipdfmx]{graphicx}
\else
  \usepackage{graphicx}
\fi

%%%
%%% Color URL
%%%
\usepackage{url}
%\usepackage[dvipdfmx]{hyperref}
\usepackage{hyperref}
%\usepackage[hidelinks,dvipdfmx]{hyperref}
\hypersetup{
    colorlinks,
    linkcolor={red!50!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black}
}
%\urlstyle{same}

%%%
%%% mediabb
%%%
% mediabb must be after graphicx? Seems not.
\usepackage{mediabb}

%%%
%%% The color package must be called AFTER the mediabb package
%%%
% Solving the inconsistencies between packages
% See for more detail: https://qiita.com/ganyariya/items/2dcb900bb04069408e14
%\usepackage[dvipdfmx]{color}
\usepackage{color}

%%%
%%% AMS math related, bold vectors
%%%
\usepackage{amsmath,amsfonts,amssymb,mathrsfs,bm,bbm}

%%%
%%% \widecheck, and more math symbols
%%% See: https://tex.stackexchange.com/questions/44235/is-there-a-way-to-do-an-upside-down-widehat
%%%
%\usepackage{mathabx}  %%% Incompatible with the PJA style?

%%%
%%% soul is used everywhere later
%%%
\usepackage{soul}

%%%
%%% Define your own colors
%%%
% Color names
% http://latexcolor.com/
% http://www.biwako.shiga-u.ac.jp/sensei/kumazawa/tex/color.html
% https://www.color-sample.com/colors/556/
 \definecolor{applegreen}{rgb}{0.55,0.71,0.0}
 \definecolor{forestgreen}{rgb}{0.13,0.55,0.13}
 \definecolor{pinegreen}{rgb}{0.0,0.47,0.44}
 \definecolor{upforestgreen}{rgb}{0.0,0.27,0.13}
 \definecolor{vividviolet}{rgb}{0.62,0.0,1.0}
 \definecolor{lightcyan}{rgb}{0.717647, 0.933071, 0.996078} % in RGB
%\definecolor{lightcyan}{cmyk}{0.280, 0.067, 0.0,   0.004}  % in CMYK
% See for the RGB pattern of Cyan, https://www.color-sample.com/colors/b7edfe/

% For \fcolorbox, see:
% http://osksn2.hep.sci.osaka-u.ac.jp/~naga/miscellaneous/tex/tex-tips4.html

%%%
%%% Use colored-boxes with linebreaks
%%%
% https://tex.stackexchange.com/questions/312574/colorbox-does-not-linebreak
%%% NOTE: You canNOT use \ctext with the \url command! (sort of conflict)
%%% But if you use \mbox, it may solve the problem:
% https://tex.stackexchange.com/questions/310817/soul-package-hl-with-cite-gives-error-citex-has-an-extra
%\usepackage{xcolor}
\newcommand{\ctext}[3][RGB]{%
  \begingroup
  \definecolor{hlcolor}{#1}{#2}\sethlcolor{hlcolor}%
  \hl{#3}%
  \endgroup
}
% \todo
 \newcommand{\todopart}[1]{{\leavevmode\ctext[RGB]{0,209,0}{#1}}}
% \revisedpart (legacy)
%\newcommand{\revisedpart}[1]{{\leavevmode\ctext[RGB]{238,232,170}{#1}}} % dark yellow
 \newcommand{\revisedpart}[1]{{\leavevmode\ctext[RGB]{183,237,254}{#1}}} % light cyan
% \revisedtext
%\newcommand{\revisedtext}[1]{{\leavevmode\textcolor{pinegreen}{#1}}}
%\newcommand{\revisedtext}[1]{{\leavevmode\textcolor{upforestgreen}{#1}}}
 \newcommand{\revisedtext}[1]{{\leavevmode\textcolor{vividviolet}{#1}}}

%%% NEW! colored revised parts (more robust)
%%% https://tex.stackexchange.com/questions/260566/how-to-reliably-switch-the-highlighting-color-with-soul
%\DeclareRobustCommand{\hlcyan}[1]{{\sethlcolor{cyan}\hl{#1}}}
%\DeclareRobustCommand{\hlcyan}[1]{{\sethlcolor{lightcyan}\hl{#1}}}
 \DeclareRobustCommand{\newrevisedpart}[1]{{\sethlcolor{lightcyan}\hl{#1}}}

%%%
%%% Do we need them? (not sure...)
%%%
%%% See for more details:
%%% https://stackoverflow.com/questions/61229757/latex-highlighting-citation-and-ref-using-different-backgrond-colors
% \newcommand{\Hl}[2][\empty]{%
% \ifx#1\empty
% \else
% \sethlcolor{#1}%
% \fi
% \hl{#2}}
%\usepackage{soul,color}
%\usepackage{soul}
\soulregister\Hl{7}
\soulregister\ref7
\soulregister\cite7
\soulregister\citet7
\soulregister\pageref7

%%%
%%% Place floats wherever you want to have it
%%% http://www.oceanwave.jp/index.php?float%B4%C4%B6%AD%28figure%2Ftable%29%A4%CE%BD%D0%CE%CF%B0%CC%C3%D6%A4%F2%A5%B3%A5%F3%A5%C8%A5%ED%A1%BC%A5%EB
%%%
\usepackage{here}

%%%
%%% To realize verbatim environment in footnotes
%%% https://tex.stackexchange.com/questions/203/how-to-obtain-verbatim-text-in-a-footnote
%%%
\usepackage{bigfoot}

%%%
%%% Temporarily for footnotes - Comment it out when submission
%%% https://tex.stackexchange.com/questions/254819/where-is-makefntext-defined
%%%
%\makeatletter
%\newcommand\@makefntext[1]{%
%    \parindent 1em%
%    \noindent
%    \hb@xt@1.8em{\hss\@makefnmark}#1}
%\makeatother

%%%
%%% BibTeX logo
%%%
\newcommand{\BibTeX}{\textsc{Bib}{\TeX}}

%%%
%%% Place as many floats as possible in each page
%%%
\renewcommand{\topfraction}{0.98}
\renewcommand{\bottomfraction}{0.98}
\renewcommand{\textfraction}{0.02}
\renewcommand{\floatpagefraction}{0.98}
\renewcommand{\dbltopfraction}{0.98}
\renewcommand{\dblfloatpagefraction}{0.98}
%%% Setting 1.0 or 0.0 can call a bug, so do not do it.
%\renewcommand{\topfraction}{1.0}
%\renewcommand{\bottomfraction}{1.0}
%\renewcommand{\textfraction}{0.00}
%\renewcommand{\floatpagefraction}{1.0}
%\renewcommand{\dbltopfraction}{1.0}
%\renewcommand{\dblfloatpagefraction}{1.0}
\setcounter{totalnumber}{50}
\setcounter{topnumber}{50}
\setcounter{bottomnumber}{50}


%%%
%%% Create and use my own counter (mailnly for the p2p response files)
%%% See: https://oshiete.goo.ne.jp/qa/9015533.html
\newcounter{revcomcounter}
\setcounter{revcomcounter}{0}
\renewcommand{\therevcomcounter}{\arabic{revcomcounter}}
\newcommand{\revcomcounter}{\refstepcounter{revcomcounter}\therevcomcounter}

%%%
%%% NatBib
%%%
\usepackage{natbib}

%%%
%%% Bibitem spacing (place after \usepackage{natbib})
%%%
% https://tex.stackexchange.com/questions/93859/condense-the-space-between-bibliographic-entries
\setlength{\bibsep}{4.5pt plus 0.25ex}

%%%
%%% eclbkbox
%%% http://konoyonohana.blog.fc2.com/blog-entry-314.html
%\usepackage{eclbkbox}

%%%
%%% Good & old ascii macro
%%%
\usepackage{ascmac}

%%%
%%% Datetime
%%% http://www.dickimaw-books.com/latex/novices/html/datetime.html
\usepackage[yyyymmdd,hhmmss]{datetime}

%%%
%%% Babel for using the Russian language environment
%%%
\usepackage[OT2,T1]{fontenc}
\usepackage[english,russian]{babel}

%%%
%%% Using more various symbols
%%% http://latextips.seesaa.net/article/449667927.html
%%%
\usepackage{textcomp}

%%%
%%% Define \erase
%%% From http://coffee.guhaw.com/Entry/637/
\usepackage{ulem}
%\DeclareRobustCommand{\erase}{\bgroup\markoverwith{\textcolor{red}{\rule[.5ex]{2pt}{0.4pt}}}\ULon}
 \DeclareRobustCommand{\erase}{\bgroup\markoverwith{\textcolor{red}{\rule[.5ex]{2pt}{1.6pt}}}\ULon}
\newcommand{\add}[1]{\textcolor{blue}{#1}}

%%%
%%% The todonotes package conflicts with something else (probably the hyperref package)
%%%
%\usepackage[colorinlistoftodos]{todonotes}
%\usepackage{todonotes}
%%%
%%% Instead, this works
%%%   for more detail: https://www.overleaf.com/learn/latex/Margin_notes
\usepackage{marginnote}
\font\srm=cmr10 at 7truept

%%%
%%% Embed ORCiD link
%%%
\usepackage{orcidlink}  % May not work with pLaTeX

%%%
%%% Using larger symbols in equations
%%%   for the detail: https://latex.org/forum/viewtopic.php?t=16899
\usepackage{relsize}

%%%
%%% Using multicolumn in the text
%%%   https://mathlandscape.com/latex-column/
%%%   https://oversleptabit.com/archives/915
%\usepackage{multicol}  %%% Incompatible with the PJA style?

%%%
%%% Wrapfigu
%%%
\usepackage{wrapfig}

%%%
%%% Used in the Kakenhi LaTeX, but often conflicts with something else
%%%
%\usepackage{okumacro}

%%%
%%% Make frames for floats
%%%   for more detail: https://tex.stackexchange.com/questions/547025/how-do-i-put-a-box-around-the-figure-and-caption-both
\usepackage{framed}

%%%
%%% Extended array
%%%
% https://okumuralab.org/tex/mod/forum/discuss.php?d=2776
% https://www.ctan.org/pkg/array
\usepackage{array}

%%%
%%% Use of colors in equations
%%% https://tex.stackexchange.com/questions/21598/how-to-color-math-symbols
%\usepackage{xcolor}
\makeatletter
\def\mathcolor#1#{\@mathcolor{#1}}
\def\@mathcolor#1#2#3{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}
\makeatother

%%%
%%% Symbols for the Moon
%%% https://tex.stackexchange.com/questions/34785/how-to-typeset-moon-phase-symbols
%%%
 \usepackage{wasysym}
 \newcommand\srM{\!\scriptsize \rightmoon}
 \newcommand\slM{\!\scriptsize \leftmoon}

%%% Symbol for the Moon
%\newcommand\msym{M}
 \newcommand\msym{\srM}  % right Moon
%\newcommand\msym{\slM}  % left  Moon

%%%
%%% Symbol for the Sun
%%%
 \newcommand\ssym{\odot}

%%%
%%% Drawing arcs
%%%   for more detail: https://tex.stackexchange.com/questions/96680/a-better-notation-to-denote-arcs-for-an-american-high-school-textbook
%%%
\makeatletter
\DeclareFontFamily{U}{tipa}{}
\DeclareFontShape{U}{tipa}{m}{n}{<->tipa10}{}
\newcommand{\arc@char}{{\usefont{U}{tipa}{m}{n}\symbol{62}}}%
\newcommand{\arc}[1]{\mathpalette\arc@arc{#1}}
\newcommand{\arc@arc}[2]{%
  \sbox0{$\m@th#1#2$}%
  \vbox{
    \hbox{\resizebox{\wd0}{\height}{\arc@char}}
    \nointerlineskip
    \box0
  }%
}
\makeatother

%%%
%%% Cancel/strikeout by slash
%%%
% https://tex.stackexchange.com/questions/40253/how-to-strike-through-obliquely-e-g-to-indicate-cancellation
\usepackage{cancel}

%%%
%%% Cancel/strikeout in a fancier way using tikz
%%%
\usepackage{tikz}
\newcommand{\hcancel}[1]{%
    \tikz[baseline=(tocancel.base)]{
        \node[inner sep=0pt,outer sep=0pt] (tocancel) {#1};
        \draw[red] (tocancel.south west) -- (tocancel.north east);
    }
}

%%%
%%% Abbreviation of journal names
%%%
\def\natauth{{\textit{Nature\/}}}
\def\natastr{{\textit{Nature Astronomy\/}}}
\def\natcomm{{\textit{Nature Communications\/}}}

%%%
%%% Equation environments
%%%
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\bea{\begin{aligned}}
\def\eea{\end{aligned}}

%%%
%%% Legacy from pream1.tex
%%%
\newcommand{\lw}[1]{\smash{\lower2.ex\hbox{#1}}}
\newcommand{\llw}[1]{\smash{\lower4.ex\hbox{#1}}}

%%%
%%% Macros for the solar system dynamics and disturbing function
%%%
\def\cosO{\cos \Omega}
\def\sinO{\sin \Omega}
\def\cosI{\cos I}
\def\sinI{\sin I}
\def\cosw{\cos \omega}
\def\sinw{\sin \omega}
\def\cosf{\cos f}
\def\sinf{\sin f}
\def\cosu{\cos u}
\def\sinu{\sin u}
\def\coslb{\cos \lambda}
\def\sinlb{\sin \lambda}

%%%
%%% Macros for the rigid body rotation
%%%
\def\bomega{\bm{\omega}}

%%%
%%% Laplace coefficient b_{#1/#2}^{(#3)} = b_s^(j)
%%%
\newcommand{\bsj}[3]{b_{\frac{#1}{#2}}^{(#3)}}

%%%
%%% Abbreviation for \begin{array}{#} and \end{array}
%%
\newcommand{\barray}[1]{\begin{array}{#1}}
\newcommand{\earray}{\end{array}}

%%%
%%% Double angles << and >>
%%%
% https://tex.stackexchange.com/questions/79657/how-to-get-double-angle-bracket-without-using-mnsymbol-package
\makeatletter
\newsavebox{\@brx}
\newcommand{\llangle}[1][]{\savebox{\@brx}{\(\m@th{#1\langle}\)}%
  \mathopen{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\newcommand{\rrangle}[1][]{\savebox{\@brx}{\(\m@th{#1\rangle}\)}%
  \mathclose{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\makeatother

%%%
%%% Poisson bracket
%%%
\newcommand{\poop}[1]{\left\{\; , \, #1\right\}}
\newcommand{\pbra}[2]{\left\{#1,\:#2\right\}}

%%%
%%% Legacy from pream3.tex
%%%   used for the translation of von Zeipel (1910)
%%%
\def\DPs#1#2#3{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\def\veps{\varepsilon}

%%%
%%% Define my own list environment
%%%
\newenvironment{mylist}[1]{%
\begin{list}{}{\setlength{\leftmargin}{#1}\setlength{\itemindent}{-#1}}}%
{\end{list}}

%%%
%%% Landscape table
%%% http://www.nemotos.net/?p=88
\usepackage{lscape}

%%%
%%% Thicker lines in the LaTeX table
%%%   http://www.geocities.co.jp/SiliconValley/7231/tabular.htm
\makeatletter
\def\Hline{%
\noalign{\ifnum0=`}\fi\hrule \@height 0.75pt \futurelet
\reserved@a\@xhline}
\makeatother

%%%
%%% "k" in the pnc font (New Century Schoolbook)
%%%
% https://w3.ual.es/~vruiz/Docencia/Apuntes/Typesetting/LaTeX/index.html#x1-310008
% http://basewall.kuciv.kyoto-u.ac.jp/dokuwiki/doku.php?id=latex#%E3%83%95%E3%82%A9%E3%83%B3%E3%83%88%E3%81%AE%E5%A4%89%E6%9B%B4%E3%83%BB%E4%B8%AD%E7%B4%9A%E8%80%85%E7%B7%A8
% https://tex.stackexchange.com/questions/88730/mathrm-or-mbox-what-is-the-convention-when-writing-a-equation
\def\ktext{\text{\usefont{T1}{pnc}{m}{it}k}}

%%%
%%% Use the ORCID logo PDF file for the ORCID ID
%%%   https://tex.stackexchange.com/questions/547843/i-get-encoding-scheme-tu-unknown-error-when-i-use-the-turkish-journal-of-ma
%%%   https://github.com/h2oai/article-information-2019/blob/master/definitions/logo-orcid-eps-converted-to.pdf
\newcommand{\orc}{\includegraphics[height=\fontcharht\font`A]{logo-orcid-eps-converted-to.pdf}}

